A General Framework for Information Extraction using Dynamic Span Graphs

We introduce a general framework for several information extraction tasks that share span representations using dynamically constructed span graphs. The graphs are constructed by selecting the most confident entity spans and linking these nodes with confidence-weighted relation types and coreferences. The dynamic span graph allows coreference and relation type confidences to propagate through the graph to iteratively refine the span representations. This is unlike previous multi-task frameworks for information extraction in which the only interaction between tasks is in the shared first-layer LSTM. Our framework significantly outperforms the state-of-the-art on multiple information extraction tasks across multiple datasets reflecting different domains. We further observe that the span enumeration approach is good at detecting nested span entities, with significant F1 score improvement on the ACE dataset.

==> 04-DWModel.tex <==
\input{figures/model_figure.tex}

\section{Model (Dave version; just trying out a few ideas)}

\paragraph{Problem Definition} The input is a document $\mathcal{D}$ represented as a sequence of words, %$D=\{w_1, \ldots, w_n\}$, 
from which we derive
$S=\{s_1,\ldots, s_N\}$, the set of all possible within-sentence word sequence spans (up to length $L$) in the document.
The output contains three structures: 
the entity types $E$ for all spans $S$, 
the relations $R$ for all span pairs $S\times S$ within the same sentence, and the coreference links $C$ for all spans in $S$ across sentences. We consider two primary tasks. First, {\it Entity recognition} is the task of predicing $E$, the entity type labels $e_i$ for each span $s_i$. Second, {\it Relation extraction} is the task of predicting $R$, the relations $r_{ij}$ for all spans $s_i$, $s_j$.
We provide additional supervision by also training our model to perform a third, auxiliary task: {\it Coreference resolution}. For this task we predict $C$, the best antecedent $c_i$ for each span $s_i$. 

\paragraph{Our Model} We develop a general information extraction framework, which we call \sys, to identify and classify entities, relations, and coreference links in a multitask fashion (sketched in Figure \ref{fig:model:mtl}). \sys\ first enumerates all text spans in each sentence, and computes a locally-contextualized vector space representation of each span. The model then employs a \emph{dynamic span graph} to incorporate global information into its span representations, as follows. At each training step, the model identifies the text spans that are most likely to represent named entities, and treats these spans as nodes in a graph structure. It constructs confidence-weighted arcs for each node according to its predicted coreferences and relations with the other nodes in the graph. It then updates the contextualized representations of all candidate entities (i.e. graph nodes) by propagating information across the arcs in the graph. In our previous multitask framework~\cite{luan2018multi}, the three learning tasks could only share information via the local span representations learned by an LSTM model. By contrast, the span graph formulation enables \sys\ to incorporate long-range dependencies captured by coreference and entity relations, iteratively refining the model's span representations. It then uses these richer, "globally contextualized" representations when making its final predictions.



\subsection{Model Architecture}

We outline the components of the \sys\ model, represented schematically in Figure \ref{fig:model:mtl}. This section provides a high-level overview. A detailed mathematical description of the dynamic span graph approach is provided in section Sec.~\ref{sec:model:graph}.


\paragraph{Token Representation Layer}

We concatenate character, GLoVe~\cite{pennington2014glove} word embeddings and ELMo embeddings \cite{peters2018deep} as model inputs. We generate locally contextualized word representations by running a bidirectional LSTm over the input and concatenating the forward and backward hidden states of the LSTM.

\paragraph{Span Representation Layer}

We construct a vector representation of each span $s_i$ by concatenating the LSTM representations of its left and right endpoints with an attention-based soft ``headword" and embedded span width
features as described in \cite{Lee2017EndtoendNC}.


\paragraph{Coreference Propagation Layer}

We construct a coreference graph using the span representations from the previous layer as input, and re-contextualize these span representations by propagating information amongst neighbors in the coreference graph. The details of this process are provided in Sec.~\ref{sec:model:graph}. We perform $N$ steps of coreference propagation, where in each step a span updates its representation by combining it with the representation of its graph neighbors. The output span representations from each step $j$ are passed as the inputs to step $j+1$. By performing $N$ steps of pairwise coreference propagation, each span can incorporate context from spans up to $N$ hops away in the coreference graph. We denote the representation of the $i^{th}$ span at step $j$ as $\mathbf{g}_i^j$.


\paragraph{Relation Propagation Layer}

The output representations of the coreference propagation layer are used as inputs by the relation propagation layer. We repeat the same process as above, except now we construct the graph based on the relations predicted by the model rather than the coreferences. The nodes update their representations based on their neighbors $M$ times, allowing for the incorporation of context from up to $M$ steps away. Since $N$ steps of coreference propagation precede relation propagation, we refer to the representation for span $i$ at iteration $j$ as $\mathbf{g}_i^{N+j}$.

\paragraph{Final Prediction Layer}

To make our final predictions for the entity labels $E$ and relations $R$, we pass the outputs of the relation propagation layer ($\mathbf{g}_i^{N+M}$) to a linear classifier to produce per-class scores, denoted as $\mathbf{p}_E (i)$ and $\mathbf{p}_R (i,j)$. We convert these scores to probabilities using the standard softmax function: $P (e_i \mid C, R, \mathcal{D}) \propto \exp (\mathbf{p}_E(i) )$
and $P (r_{ij} \mid C, \mathcal{D}) \propto \exp (\mathbf{p}_R (i,j))$. 
The coreference scores are normalized by maximizing the score of gold antecedent over all candidate antecedents in the coreference beam.

%\subsection{Span Representation Refinement through Dynamic Graph Construction}
\subsection{Dynamic Graph Construction and Span Refinement}
\label{sec:model:graph}
 The  span graph facilitates propagating broader context through soft coreference and relation links to update span representations.  \luanyi{changed higher order to broader context}.
 The nodes in the span graph consist of spans $s_i$ with vector representations $\mathbf{g}^n_i \in \mathbb{R}^{d} $. The edges between spans are weighted according to the coreference and relation scores, which are trained according to the neural architecture explained in Section~\ref{sec:model_architecture}. In the following we explain how coreference and relation links can update span representations.  
 
 \paragraph{Coreference Propagation} For the whole document, we define a beam consisting of $b_c$ spans that are most likely to be in a coreference chain.  We consider $\mathbf{P}_C^n$ to be a matrix of real values that indicate coreference confidence scores between these spans in the $n$-th iteration. $\mathbf{P}_C^n$ is of size $b_c \times K$, where $K$ is the maximum number of antecedents considered. For the coreference graph, an edge in the graph is single directional, connectinf the current  span $s_i$ with all its potential antecedents $s_j$ in the coreference beam, where $j < i$.  The edge between two nodes $s_i$ and $s_j$ are weighted according to the coreference confidence score $P^n_C(i,j)$. 
The following equation shows how the coreference context span representation $\mathbf{u}_i^{C}\in \mathbb{R}^{d}$ is computed by propagating the co-referred span representations $\mathbf{g}_j^{n}$ weighted by their coreference scores  $P_C^n(i,j)$. %are refined given the n each graph layer, we get the updated span embedding $\mathbf{a}_i^{n}$ through the following function:
\begin{equation} \label{eq:coref}
 \mathbf{u}_C^n(i)=  \sum_{j\in B_\text{C}(i)} P^n_C(i,j)\mathbf{g}_j^{n}
\end{equation}
where $B_C(i)$ is the set of $K$ spans that are antecedents of $s_i$, 
\begin{equation}
    P_C^n(i,j) = \frac{
    \exp(V_C^n(i,j))}{ \sum_{j' \in \mathcal{Y}(i)} \exp(V_{C}^n(i,j))}
\end{equation}
and $V_C^n(i,j)$ is a feedforward network score taking $\mathbf{g}_i^n$ and $\mathbf{g}_j^n$ as input. 
%% maybe include equation or cite previous paper

\mo{There remains a question of whether to use boldface for $V_c$ and $V_R$ and/or $P$. It is inconsistent here since we weren't sure which way to go.}

\paragraph{Relation Propagation}  For each sentence, we define a beam $B_R$ consisting of $b_r$ entity spans that are mostly likely to be involved in a relation.  Unlike coreference graph, the weights of relation edges capture different relation types.  Therefore for the $n$-th iteration, we use a tensor $\mathbf{V}_R^{n}\in \mathbb{R}^{b_R\times b_R \times L_R} $ that captures scores of each of the $L_R$ relation types. 
In other words, the edges in the graph connect two entity spans $s_i$ and $s_j$ in the relation beam according to  the $L_R$-length vector of predicted relation scores $\mathbf{V}_R^n(i,j)$, which is computed using a feedforward network taking $g_i^n$ and $g_j^n$ as inputs. 
%% maybe include equation or cite paper
The following equation shows how the relation context span representation  $\mathbf{u}^n_{R}(i)\in \mathbb{R}^{d}$ is updated by propagating span representations: 
\begin{align}\label{eq:relation}
 \mathbf{u}^n_{R}(i) =  \sum_{j\in B_\text{R}} f(\mathbf{V}^n_R(i,j))\mathbf{A}_R \odot \mathbf{g}_j^{n}, 
\end{align}
where $\mathbf{A}_R \in \mathbb{R}^{L_R\times d}$ is a trainable linear projection matrix, 
$f$ is a non-linear function to select the most important relations, and $\odot$ is element-wise multiplication. Due to the fact that only a small number of entities in the relation beam have the actual relationship with the target span, connecting edges between all possible span pairs would introduce lots of noise to the new representation.
Therefore, we choose $f$ to be the ReLU function to removes the effect of unlikely relations by setting the dimension of negative relation scores to 0.
Unlike corefence connections, two spans linked via a relation are not expected to have similar representations, so the matrix $\mathbf{A}_R$ helps to transform the embedding $\textbf{g}_j^n$ according to each relation type.  

\paragraph{Updating Span Representations with Gating} In order to compute the new span representations, we define a gating vector $\mathbf{f}_i^{x}\in \mathbb{R}^{d}$, where $x\in\{C,R\}$ to determine whether to keep the previous span representation $\mathbf{g}_i^{n}$ or to integrate new information from coreference or relation context span representation $\mathbf{u}^n_{x}(i)$. More formally, 
\begin{eqnarray}
\mathbf{f}_x^n(i) &=& g(\mathbf{W}^{\text{f}}_x[\mathbf{g}_i^{n},\mathbf{u}^n_{x}(i)]) \label{eq:gate}\\
\mathbf{g}_i^{n+1} &=& \mathbf{f}_x^n(i)\odot \mathbf{g}_i^{n} + (1-\mathbf{f}_x^n(i)) \odot \mathbf{u}^n_x(i) \notag
\end{eqnarray}
% \hanna{for ui and fi, you don't need to have the superscript n, right? I am adding superscript X, where X is either R or C}
% \hanna{This shouldn't be Wx, we already have used WR.} \hanna{don't do sigma, do g, and in the implementation details or in the text say you used sigmoid}
where $\mathbf{W}^{\text{f}}_x \in \mathbb{R}^{d\times 2d}$ is a trainable parameter for the gating function. Here, $g$ is the element-wise sigmoid function.
% \hanna{The iterations in the propagations are not explained -- maybe this can be deferred to the model architecture} 

\subsection{Training}

The loss function is defined as a weighted sum of the  log-likelihood of all three tasks:
\begin{align}
    %\mathcal{J}(R^*, E^*, C^*, D) =& 
 & \sum_{(D, R^*, E^*, C^*) \in\mathcal{D}} \Big\{ 
 \lambda_{\text{E}}\log P (E^* \mid C, R, \mathcal{D})   \\
 & + \lambda_{\text{R}}\log P (R^* \mid C, \mathcal{D}) + \lambda_{\text{C}}\log P (C^* \mid \mathcal{D}) \Big\}\notag
\end{align}
where $E^*$, $R^*$ and $C^*$ are gold structures of the entity types, relations and coreference respectively.
The task weights $\lambda_{\text{E}}$, $\lambda_{\text{R}}$, and $\lambda_{\text{C}}$ are introduced as hyper-parameters to control the importance of each task.
\luanyi{mention coref data doesn't have be overlapped annotations, and we use coreference as an auxiliary task}

\mo{ move implementation details here}


==> 04-OldModel.tex <==
\input{figures/model_figure.tex}

\section{Model}


\subsection{Overview}
\paragraph{Problem Definition} The input is a document represented as a sequence of words $\mathcal{D}$, %$D=\{w_1, \ldots, w_n\}$, 
from which we derive
$S=\{s_1,\ldots, s_N\}$, the set of all possible within-sentence word sequence spans (up to length $L$) in the document.
The output contains three structures: 
the entity types $E$ for all spans $S$, 
the relations $R$ for all span pairs $S\times S$ within the same sentence, and the coreference links $C$ for all spans in $S$ across sentences.  
 In particular, {\it Entity recognition} is to predict the best entity type $e_i$ for every candidate span $s_i$. {\it Relation extraction} is to predict  the best relation type $r_{ij}$ given an ordered pair of spans $(s_i,s_j)$. {\it Coreference resolution} is to predict the best antecedent $c_i$  given a span $s_i$. 


\paragraph{Our Model} We develop a general information extraction framework (called \sys) to identify and classify  entities, relations, and coreference in a multi-task setup (sketeched in Figure \ref{fig:model:mtl}). \sys\  enumerates all phrase spans in a sentence, encodes them in a vector space representation through local context, and refines the span representations using global information by propagating the entity and relation type confidences through a {\it graph of spans}. At each  training step, the graph of spans are dynamically constructed by selecting the most confident entity spans and linking these nodes with confidence-weighted relation types and coreferences.  Then, the span representations are refined using global context from  propagations of  neighboring relation types and corefered entities.  Unlike the previous multi-task framework~\cite{luan2018multi} in which the only interaction between tasks is the shared first-layer LSTM capturing local context, our model uses the global context through the span graph to  allow entity and relation type confidences to propagate through the graph to iteratively refine the result. The refined span representations are used in a multi-task framework to predict entity types, relation types, and coreference links. \hanna{I think an example would help here -- or referring back to the figure}


 

\subsection{Span Representation Refinement through Dynamic Graph Construction}
 The  span graph facilitates propagating broader context through soft coreference and relation links to update span representations.  \luanyi{changed higher order to broader context}.
 The nodes in the span graph consist of spans $s_i$ with vector representations $\mathbf{g}_i \in \mathbb{R}^{d} $. The edges between spans are weighted according to the coreference and relation scores, which are trained according to the neural architecture explained in Section~\ref{sec:model_architecture}. In the following we explain how coreference and relation links can update span representations.  
 
 
 \paragraph{Coreference Propagation} For the whole document, we define a beam $B_C$ consisting of $b_c$ spans that are most likely to be coreference mentions.  We consider $\mathbf{P}_C^n$ to be a matrix of real values that indicate coreference confidence scores in the $n$-th iteration. $\mathbf{P}_C^n$ is of size $b_c \times b_c$. For the coreference graph,  the edges in the graph is single directional which connect the current  span $s_i$ with all its potential antecedents $s_j$ in the coreference beam, where $j < i$.  The edge between two nodes $s_i$ and $s_j$ are weighted according to the coreference confidence score $P^n_C(i,j)$. 
The following equation shows how the coreference context span representation $\mathbf{u}_i^{C}$ is computed by propagating the co-referred span representations $\mathbf{g}_j^{n}$ weighted by their coreference scores  $P_C^n(i,j)$. %are refined given the n each graph layer, we get the updated span embedding $\mathbf{a}_i^{n}$ through the following function:
\begin{equation} \label{eq:coref}
 \mathbf{u}_i^C =  \sum_{j\in B_\text{C}} P^n_C(i,j)\cdot \mathbf{g}_j^{n} 
\end{equation}

\luanyi{not sure if $\mathbf{P}$ is going to be misleading, since $\mathbf{P}$ is not probability, but scores of real values} \luheng{Maybe? Also I'm a bit confused by the direction of coreference links here. Is $P$ defined for all pairs in the beam, or just (mention, antecedent pairs) (where $j \leq i$?). In general I was just wondering if you treat coreference links as directed.}

\paragraph{Relation Propagation}  For each sentence, we define a beam $B_R$ consisting of $b_r$ candidate entity spans that are mostly likely to be involved in a relation.  Unlike coreference graph, the weights of relation edges capture different relation types.  Therefore for the $n$-th iteration, we use a tensor $\mathbf{P}_R^{n}$ of real value that captures relation confidences of each relation type. $\mathbf{P}_R^{n}$ has size $b_r \times b_r \times L_R$, where $L_R$ indicates the number of relation types.
For the relation graph,  the edges in the graph connect two entity spans $s_i$ and $s_j$ in the relation beam according to  the predicted relation scores $\mathbf{p}_R^n(i,j)$, which is a vector of size $L_R$ indicating the confidence score of each relation type. \luanyi{maybe redundant, not sure about the notation of $\mathbf{p}_R^n(i,j)$ as a vector.}
The following equation shows how the relation context span representation  $\mathbf{u}_i^{R}$ is affected by propagating span representations from the neighboring spans. 

\begin{align*}\label{eq:relation}
 \mathbf{u}_i^{R} =  \sum_{j\in B_\text{R}} f(\mathbf{p}^n_R(i,j))\cdot  \mathbf{W}_R \odot \mathbf{g}_j^{n}, 
\end{align*}
where $\mathbf{W}_R \in \mathbb{R}^{L_R\times d}$ is a trainable relation transformation matrix \luheng{or just: linear projection matrix?},  
% $d$ indicates the dimension of span representation $\mathbf{g}_i^n$, 
$f$ is a non-linear function to select the most important relations. Due to the fact that only a small number of entities in the relation beam have the actual relationship with the target span, connecting edges between all possible span pairs would introduce lots of noise to the new representation.
Therefore, we choose $f$ to be the ReLU function  that  removes the effect of null-type relation and prune out unconfident edges by setting the dimension of negative relation scores  to 0. \hanna{why just null-type? -- better explanation here} \luanyi{explained, maybe need rewording} \luheng{we might need to mention the 0 NULL score thing in 2.1 overview so it's not an information overload here.} The matrix $\mathbf{W}_R$ helps to transform the embedding $\textbf{g}_j^n$ according to each relation type confidence scores between span pairs. \luheng{Ppl might wonder why you used a scalar weight for coref and a vector weight for relation, is there a natural explanation for this? Basically $f(\mathbf{p}_R(i,j))\cdot W_R$ can be think of as a ``vectorized weight'', right?}
\hanna{I agree with Luheng, it would be good if you use the same formulation...we can vectorize for coref as well}

\paragraph{Updating Span Representations with Gating} In order to compute the new span representations, we define a gating vector $\mathbf{f}_i^{X}$, where $X\in\{C,R\}$ to determine whether to keep the previous span representation $\mathbf{g}_i^{n}$ or to integrate new information from coreference or relation context span representation $\mathbf{u}_i^{X}$. More formally, 
\begin{eqnarray}
\mathbf{f}_i^{X} &=& g(\mathbf{W}_{\text{f}}^X[\mathbf{g}_i^{n},\mathbf{u}_i^{X}]) \label{eq:gate}\\
\mathbf{g}_i^{n+1} &=& \mathbf{f}_i^{X} \odot \mathbf{g}_i^{n} + (1-\mathbf{f}_i^{X}) \odot \mathbf{u}_i^{X} \notag
\end{eqnarray}
% \hanna{for ui and fi, you don't need to have the superscript n, right? I am adding superscript X, where X is either R or C}
% \hanna{This shouldn't be Wx, we already have used WR.} \hanna{don't do sigma, do g, and in the implementation details or in the text say you used sigmoid}
where $\mathbf{W}_{\text{f}}^X$ is a trainable parameter for the gating function. $g$ is the element-wise sigmoid function.
\luanyi{use $\mathbf{W}_{\text{f}}^X$ for gating params, not explaining iteration process in this section}
% \hanna{The iterations in the propagations are not explained -- maybe this can be deferred to the model architecture} 

\subsection{Model Architecture}
\label{sec:model_architecture}
%We develop a general information extraction framework (called \sys) to identify and classify scientific entities, relations, and coreference. Unlike the baseline model ~\cite{luan2018multi} in which the only interaction between tasks is the shared first-layer LSTM, the dynamic span graph allows entity and relation type confidences to propagate through the graph to iteratively refine the result. 
\sys\ consists of the following components and layers. Figure \ref{fig:model:mtl} shows a high-level overview of the \sys\ framework. 


\paragraph{Token Representation Layer}
We apply a bidirectional LSTM at the token level taking the concatenated character, GLoVe~\cite{pennington2014glove} word embeddings and ELMo embeddings \cite{peters2018deep} as input. The token representation is obtained by stacking the forward and backward LSTM hidden states.

\paragraph{Span Representation Layer}
For a span $s_i$, its vector representation $\mathbf{g}_i$ is constructed by concatenating the left and right end points of $s_i$ from the BiLSTM outputs, an attention-based soft ``headword", and embedded span width
features, following \cite{Lee2017EndtoendNC}.


\paragraph{Coreference Propagation Layer}
The span embedding from span enumeration layer is used to initialize the span representation at $\mathbf{g}_i^1$. 
At each iteration $n$, we first compute the expected span representation $\mathbf{u}_i^{C}$ of each span $s_i$  according to the equation \ref{eq:coref}. We then update the new span representation $\mathbf{g}_i^{n+1}$ by learning the gating vector $\mathbf{f}_i^C$ according to the equation $\ref{eq:gate}$.  By iterating this process $N$ times, the final span representation $\mathbf{g}_i^{N}$ includes higher order captures information from antecedents that are further in the document. \luanyi{This is really the same process as Kenton, we probably don't want to overclaim it.} % learn the gating function $f_i^n$ according to the equation  by using the current antecedent distribution $P(c_i = j|D)$ as an attention mechanism through Eq.~\ref{eq:link} and ~\ref{eq:gate}, where $\text{Link}_C(i, j,  \mathbf{g}_j^{n})$ is defined as:
%\begin{equation}
% \text{Link}_C(i, j,  \mathbf{g}_j^{n}, B_\text{C}) = \sum_{j\in B_\text{C}} P(c_i = j|D) \cdot \mathbf{g}_j^{n}
%\end{equation}

\paragraph{Relation Propagation Layer}
The relation propagation layer is initialized by updated representation from  coreference propagation layer $\mathbf{g}_i^{N}$.  At each iteration $n$, we first compute the expected span representation $\mathbf{u}_i^{R}$ of each span $s_i$  according to the equation \ref{eq:relation}. We then update the new span representation $g_i^{n+1}$ by learning the gating function $\mathbf{f}_i^n$ according to the equation $\ref{eq:gate}$. Information can be integrated from multiple relation paths by iterate this process $M$ times. This can be regarded as capturing information of walking $M$ steps in a relational graph, which have been commonly used for knowledge graph reasoning.  \luanyi{cite TransE or any link prediction paper. Not sure if this claim makes sense.} 
%On the $n$-th iteration, we connect the within sentence candidate span pairs in the relation beam $B_R$ through the predicted relation scores ${\mathbf P^R_{ij}}$, which is a vector of real values indicating the confidence score of each relation type. %$ $\Phi_{\text{R}}^n(s_i, s_j) \in \mathbb{R}^{L_R}$ and update the span embedding $\mathbf{g}_i^{n}$ using Eq.~\ref{eq:link} and ~\ref{eq:gate}. 
%We introduce a trainable relation transformation matrix $\mathbf{W}_R \in \mathbb{R}^{L_R\times d}$, where $L_R$ indicates number of relation types and $d$ indicates the dimension of span representation $\mathbf{g}_i^n$.
% The relation graph link function $\text{Link}_R(i, j,  \mathbf{g}_j^{n}, B_R)$ is defined as follows:

%\begin{align}
%&\text{Link}_R(i, j,  \mathbf{g}_j^{n}, B_R) = \\
%&\sum_{j\in B_\text{R}} \text{ReLU}(\Phi_{\text{R}}(s_i, s_j)) \cdot \mathbf{W}_R  \odot \mathbf{g}_j^{n}
%\end{align}
%where, we first take a ReLU  of the relation scoring function $\text{ReLU}(\Phi_{\text{R}}(r, s_i, s_j))$  that can remove the effect of null-type relation by setting the dimension of negative relation scores  to 0. 
%We then transform the embedding of $s_j$ through relation transform matrix $\mathbf{W}_R$, which can efficiently capture the relationship between span pairs. By iterating this updating process $M$ times,  candidate entity spans are connected through the relation graph, which allows information to interact through multiple relation paths. \luanyi{This is similar to knowledge graph reasoning process.}


\subsection{Training}
\paragraph{Objective function}
\luheng{Another trick to make things more clear is to use ``text'' for super/subscripts of names, and regular math font for variables e.g. $\mathbf{p}^n_{\text{R}}$ because here $\text{R}$ stands for ``relation'' and is not a variable.}
\luanyi{Concerns of this section after talking to luheng: 1, we never mention how we get $\mathbf{P}_R$ and $\mathbf{P}_C$ until here, which would be very hard to understand for people who haven't read our previous paper. 2, we probably need to mention scores $<0$  are pruned while 
$>0$ means confidence scale}
Given the input document $\mathcal{D}$, we use the final representation updated by coreference and relation graph layer $\mathbf{g}_i^{N+M}$
to predict entity $E$ and relation $R$. For entity and relation, we pass $\mathbf{g}_i^{N+M}$ to a linear classifier to produce per-class scores $\mathbf{p}_E (i)$ and $\mathbf{p}_R (i,j)$ for token $i$. We compute locally normalized probabilities for entity and relation using the softmax function: $P (e_i \mid C, R, \mathcal{D}) \propto \exp (\mathbf{p}_E(i) )$
and $P (r_{ij} \mid C, \mathcal{D}) \propto \exp (\mathbf{p}_R (i,j))$. \luanyi{we should really find a better notation for scoring functions $\mathbf{p}_E (i)$ and $\mathbf{p}_R (i,j)$, }. \luheng{So if we use another letter for ``spans'', we will be able to use $\mathbf{s}$ for all the scores ... :) we can also use greek letters such as $\phi$ ...}
Coreference is normalized by maximizing the score of gold antecedent over all candidate antecedents in the coreference beam. \luanyi{do we still need the equation for coref?} \luheng{It's good to write them concretely for now to make sure everything is consistent. We can always prune them or move them to supplementary later.}
\begin{align}
    P(c_{i}=j\mid D) = \frac{
    \exp(P_C(s_i, s_j))}{ \sum_{j' \in \mathcal{Y}(i)} \exp(P_{C}(s_{i}, s_{j'}))}
\end{align}

The loss function is defined as a weighted sum of the  log-likelihood of all three tasks:
\begin{align}
    %\mathcal{J}(R^*, E^*, C^*, D) =& 
 & \sum_{(D, R^*, E^*, C^*) \in\mathcal{D}} \Big\{ 
 \lambda_{\text{E}}\log P (E^* \mid C, R, \mathcal{D})   \\
 & + \lambda_{\text{R}}\log P (R^* \mid C, \mathcal{D}) + \lambda_{\text{C}}\log P (C^* \mid \mathcal{D}) \Big\}\notag
\end{align}

where $E^*$, $R^*$ and $C^*$ are gold structures of the entity types, relations and coreference respectively.
The task weights $\lambda_{\text{E}}$, $\lambda_{\text{R}}$, and $\lambda_{\text{C}}$ are introduced as hyper-parameters to control the importance of each task.
\luanyi{mention coref data doesn't have be overlapped annotations, and we use coreference as an auxiliary task}

% The conditional probabilities of each random variable are independently normalized: $P (E^* \mid C, R, D) \propto$
% \begin{align}
% \label{eq:normalizer}
%     & P(e_{i}=e\mid D) = \frac{
%         \exp(\Phi_{\text{E}}(e, s_i))}{ \sum_{e'\in L_{\text{E}}} 
%         \exp(\Phi_{\text{E}}(e', s_i))}  \\  
%     & P(r_{ij}=r\mid D) = \frac{
%         \exp(\Phi_{\text{R}}(r, s_i, s_j))}{ \sum_{r'\in L_{\text{R}}} 
%         \exp(\Phi_{\text{R}}(r', s_i, s_j))}  \notag \\
%     & P(c_{i}=j\mid D) = \frac{
%         \exp(\Phi_{\text{C}}(s_i, s_j))}{ \sum_{j' \in \mathcal{Y}(i)} \exp(\Phi_{\text{C}}(s_{i}, s_{j'}))}, \notag
% \end{align}
% where $\Phi_{\text{E}}$ denotes the unnormalized model score for an entity type $e$ and a span $s_i$, $\Phi_{\text{R}}$ denotes the score for a relation type $r$ and span pairs $s_i, s_j$, and $\Phi_{\text{R}}$ denotes the score for a binary coreference link between $s_i$ and $s_j$. We follow the same scoring function $\Phi_{\text{E}}$, $\Phi_{\text{R}}$ and $\Phi_{\text{C}}$ as \newcite{luan2018multi}.



% For entity recognition and relation extraction, $P(E^*\mid D)$ and $P(R^*\mid D)$ are computed with the definition in Equation \eqref{eq:decompose}.
% For coreference resolution, we use the marginalized loss following \newcite{Lee2017EndtoendNC} since each mention can have multiple correct antecedents. Let $C^*_i$ be the set of all correct antecedents for span $i$, we have:
%      $\log P (C^* \mid D)  = \sum_{i=1..N} \log \sum_{c\in C^*_i} P(c \mid D)$. %  \label{eq:coref_loss}
%\end{align}
%\hanna{why did we separate coref only here? how about the other two tasks} 
%\luheng{only coref uses marginalized loss}









% \subsection{Scoring Architecture}\label{sec:model:scoring}
% We use feedforward neural networks (FFNNs) over \emph{shared span representations} $\mathbf{g}$ to compute a set of span and pairwise span scores. 
% For the span scores, $\phi_e(s_i)$ measures how likely a span $s_i$ has an entity type $e$, and $\phi_{\text{mr}}(s_i)$ and $\phi_{\text{mc}}(s_i)$ measure how likely a span $s_i$ is a mention in a relation or a coreference link, respectively. The pairwise scores $\phi_r(s_i, s_j)$ and $\phi_{\text{c}}(s_i, s_j)$ measure how likely two spans are associated in a relation $r$ or a coreference link, respectively. 
% Let $\mathbf{g}_i$ be the fixed-length vector representation for span $s_i$.
% For different tasks, the span scores $\phi_{\text{x}}(s_i)$ for $\text{x} \in \{e, \text{mc}, \text{mr}\}$ and pairwise span scores $\phi_{\text{y}}(s_i,s_j)$ for $\text{y} \in \{ r, \text{c}\}$ are computed as follows:
% \begin{align*}
%      \phi_{\text{x}} (s_i) =& \mathbf{w}_{\text{x}} \cdot \text{FFNN}_{\text{x}} (\mathbf{g}_i) \\
%      \phi_{\text{y}} (s_i, s_j) =& \mathbf{w}_{\text{y}}\cdot \text{FFNN}_{\text{y}} ([
%         \mathbf{g}_i, \mathbf{g}_j, \mathbf{g}_i \odot \mathbf{g}_j]),
% \end{align*}
% where $\odot$ is element-wise multiplication, and $\{ \mathbf{w}_{\text{x}}, \mathbf{w}_{\text{y}}\}$ are neural network parameters to be learned. 

% We use these scores to compute the different $\Phi$:
% \begin{eqnarray}
%  \Phi_{\text{E}}(e, s_i) &= &\phi_{e}(s_i) \label{eq:factors} \\
%  \Phi_{\text{R}}(r, s_i, s_j) &= & % \nonumber\\ 
% \phi_{\text{mr}}(s_i) + \phi_{\text{mr}}(s_j)  + \phi_{r}(s_i, s_j) \notag \\
%  \Phi_{\text{C}}(s_i, s_j) &=& \phi_{\text{mc}}(s_i) + %\notag\\ 
%  \phi_{\text{mc}}(s_j) + \phi_{\text{c}}(s_i, s_j) \notag 
% %\;\;e,r,j\neq \epsilon \notag
% \end{eqnarray}

% The scores in Equation \eqref{eq:factors} are defined for entity types, relations, and antecedents that are not the null-type $\epsilon$.
% Scores involving the null label are set to a constant 0:
% $ \Phi_{\text{E}}(\epsilon, s_i)=\Phi_{\text{R}}(\epsilon, s_i, s_j)=\Phi_{\text{C}}(s_i,\epsilon)=0$. 

% We use the same span representations $\mathbf{g}$ from \cite{Lee2017EndtoendNC}
% and share them across the three tasks.
% We start by building bi-directional LSTMs \cite{hochreiter1997long} from word, character and ELMo \cite{peters2018deep} embeddings. 

% For a span $s_i$, its vector representation $\mathbf{g}_i$ is constructed by concatenating $s_i$'s left and right end points from the BiLSTM outputs, an attention-based soft ``headword,'' and embedded span width features.
% Hyperparameters and other implementation details will be described in Section \ref{sec:exp_setup}.

% \subsection{Inference and Pruning}
% Following previous work, we use beam pruning to reduce the number of pairwise span factors from $O(n^4)$ to $O(n^2)$ at both training and test time, where $n$ is the number of words in the document.
% We define two separate beams: $B_{\text{C}}$ to prune spans for the coreference resolution task, and $B_{\text{R}}$ for relation extraction. The spans in the beams are sorted by their span scores $\phi_{\text{mc}}$ and $\phi_{\text{mr}}$ respectively, and the sizes of the beams are limited by $\lambda_{\text{C}} n$ and $\lambda_{\text{R}} n$. 
% We also limit the maximum width of spans to a fixed number $W$, which further reduces the number of span factors to $O(n)$.

==> 08-Tables.tex <==
% Table dump. These will go in their own sections, but for now I'll put them all here.

% Data summary

Summary of data blah blah

\begin{table}[t]
\centering
{\footnotesize
\begin{tabular}{lllrrr}
\toprule
& Domain & Split from & ner labels & rel labels & corpus size \\
\midrule
ACE-2004 non-overlapping & newswire & \cite{li2014incremental} & 7 & 7 & 348 \\
ACE-2004 overlapping & newswire & \cite{Lu2015JointME} & 7 & 7 & 443 \\
ACE-2005 non-overlapping & newswire & \cite{li2014incremental} & 7 & 6 & 511 \\
ACE-2005 overlapping & newswire & \cite{Lu2015JointME} & 7 & 6 & 437 \\
GENIA & biomedical & \cite{Wang2018NeuralSH} & 5 & - & 1999 \\
Wet Lab Protocols & experimental process & \cite{Kulkarni2018AnAC} & 18 & 13 & 622 \\
\bottomrule
\end{tabular}
}
\caption{Summary of data sets}
\end{table}

% Results summary

Summary of results blah blah

\begin{table}[t]
\centering
{\footnotesize

\begin{tabular}{llrrrr}
\toprule
Task & Previous SOTA paper & Previous SOTA & DynGraph & Absolute change & Relative change \\
\midrule
Ace 2004 non-overlapping NER & \cite{miwa2016end} & 81.8 & - & - & - \\
Ace 2004 non-overlapping REL & \cite{miwa2016end} & 48.4 & - & - & - \\
Ace 2004 overlapping NER & \cite{Wang2018NeuralSH} & 75.1 & - & - & - \\
Ace 2005 non-overlapping NER & \cite{zhang2017end} & 83.6 & 88.4 & 4.8 & - \\
Ace 2005 non-overlapping REL & \cite{zhang2017end} & 57.5 & 63.2 & 5.7 & - \\
Ace 2005 overlapping NER & \cite{Wang2018NeuralSH} & 74.5 & 82.9 & 8.4 & - \\
GENIA overlapping NER & \cite{Wang2018NeuralSH} & 75.1 & - & - & - \\
Wet Lab NER & \cite{Kulkarni2018AnAC} & 78.03 & - & - & - \\
Wet Lab REL & \cite{Kulkarni2018AnAC} & 54.85* & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Results}
\end{table}

==> GraphProp.tex <==
\section{Dynamic Entity Graph Propagation}
 Inspired by \cite{lee2018higher}, where higher-order inference improves coreference resolution, we propose a Dynamic Entity Graph (DEG) module that can propagate information through soft coreference and relation links  to improve entity and relation extraction tasks. 
 A common component used throughout the model is the vector representations $\mathbf{g}_i$ for each possible span $i$. DEG involves $N$ iterations of refining span representations based on coreference predictions, denoted as $\mathbf{g}_i^{n}$, followed by $M$ iterations based on relation predictions, denoted as $\mathbf{g}_i^{m}$.   $\mathbf{g}_i^{n}$ starts with the span representation in the baseline model. 
 $\mathbf{g}_i^{m}$ starts with $\mathbf{g}_i^{N}$.

\subsection{Coreference Propagation}
At each iteration, we first compute the expected antecedent representation $\mathbf{a}_i^{n}$ of each span $i$ by using the current antecedent distribution $P(c_i = j|D)$ as an attention mechanism:
\begin{equation}
\mathbf{a}_i^{n} = \sum_{j\in \mathcal{Y}(i)} P(c_i = j|D) \cdot \mathbf{g}_j^{n}
\end{equation}

\noindent where for each span $s_i$ all preceding spans are $\mathcal{Y}(i) \in \{1,\ldots,i-1,\epsilon\}$. \luheng{There seem to be some inconsistency with the relation propagation model. Did you use all ``preceding spans'' or just the coref beam? We can also define a ``soft link function'', where
$\mathbf{a}_i^{n} = \sum_{j\in B} \text{Link}(i, j, \ldots) \odot \mathbf{g}_j^{n}$, and define them separately for coref and relations. This way you can reuse the equations in coref and relation propagation, and make the algorithm seem more general.} \luanyi{just the coref beam. totally agree, will work on it} The current span representation $\mathbf{g}_i^{n}$ is then updated via interpolation with its expected antecedent representation $\mathbf{a}_i^{n}$:
\begin{eqnarray}
\mathbf{f}_i^{n} &=& \sigma(\mathbf{W}_{fc}[\mathbf{g}_i^{n},\mathbf{a}_i^{n}])\\
\mathbf{g}_i^{n+1} &=& \mathbf{f}_i^{n} \odot \mathbf{g}_i^{n} + (1-\mathbf{f}_i^{n}) \odot \mathbf{a}_i^{n}
\end{eqnarray}

The learned gate vector $\mathbf{f}_i^{n}$ determines for each dimension whether to integrate new information from its expected antecedent. At iteration $n$, $\mathbf{g}_i^{n}$ is an element-wise weighted average of all expected antecedents $c_i$, controlled by coreference confidence $P(c_i = j|D)$, allowing information to flow from confident antecedents to span $s_i$ softly. By iterating this process $n > 1$ times, the current span representation $\mathbf{g}_i^{n}$  is able to get information from antecedents that are further ahead in the document.

\subsection{Relation Propagation}
In the work of \newcite{christopoulou2018walk},  all the entities in a sentence are placed as nodes in fully-connected graph structure. Since \newcite{christopoulou2018walk} assumes entities are given beforehead, they have nodes fixed in their graph. However, in our model, since we are predicting entities and relation jointly, the node of the graph changes dynamically based on the entity candidates in the relation beam. Furthermore, relation types are not considered in \newcite{christopoulou2018walk}, where entity pairs with different relation types are treated equally in the graph.  Based on this observation, we incorperate previous work of TransE model \luanyi{cite TransE and some link prediction work}, we introduce an relation transformation vector $w_r$ for each relation type and construct the graph dynamically based on the predicted relation scores $\Phi_{\text{R}}(r, s_i, s_j)$ \luanyi{Maybe move this paragraph to related work. }

The start of relation propagation starts from the updated representation of the last coreference iteration ($m$ starts from $n$). At each relation iteration, in order to get an updated embedding for the target span $s_i$, we first take a ReLU (denoted as $\sigma$) of the relation scoring function $\sigma(\Phi_{\text{R}}(r, s_i, s_j))$. \luheng{Maybe just use \text{ReLU}? $\sigma$ always reminds me of sigmoid ..} The ReLu function can efficiently remove the effect of null-type relation by setting the negative relation scores of $\Phi_{\text{R}}(r, s_i, s_j)$ to 0. We then transform the embedding of $s_j$ through relation transform vector $\mathbf{w}_r$ \luheng{maybe give a more intuitive explanation of the ``relation transform vector'', and specify its dimensions.}, where $s_j$ can be any other spans in the relation beam $B_\text{R}$. The equation is as follows:
\begin{equation}
\mathbf{b}_i^{m} = \sum_{j\in B_\text{R}} \sigma(\Phi_{\text{R}}(r, s_i, s_j)) \cdot \mathbf{w}_r  \odot \mathbf{g}_j^{m-1}
\end{equation}


\begin{eqnarray}
\mathbf{f}_i^{m} &=& \sigma(\mathbf{W}_{fr}[\mathbf{g}_i^{m},\mathbf{b}_i^{m}])\\
\mathbf{g}_i^{m+1} &=& \mathbf{f}_i^{m} \odot \mathbf{g}_i^{m} + (1-\mathbf{f}_i^{m}) \odot \mathbf{b}_i^{m}
\end{eqnarray}






==> S01-AnnotationGuideline.tex <==
% \section{Introduction}
\section{Annotation Guideline}
\label{sec:annotation}

\subsection{Entity Category}

 \begin{itemize}
\item \textbf{Task}: Applications, problems to solve, systems to construct.

E.g. information extraction, machine reading system, image segmentation, etc.

\item \textbf{Method}: Methods , models, systems to use, or tools, components of a system, frameworks. 

E.g. language model, CORENLP, POS parser, kernel method, etc.

\item \textbf{Evaluation Metric}: Metrics, measures, or entities that can express quality of a system/method. 

E.g. F1, BLEU, Precision, Recall, ROC curve, mean reciprocal rank, mean-squared error, robustness, time complexity, etc.

\item \textbf{Material}: Data, datasets, resources, Corpus, Knowledge base.

E.g. image data, speech data, stereo images, bilingual dictionary, paraphrased questions, CoNLL, Panntreebank, WordNet, Wikipedia, etc.

\item \textbf{Evaluation Metric}: Metric， measure， or term that can express quality of a system/method.

E.g. F1, BLEU, Precision, Recall, ROC curve, mean reciprocal rank, mean-squared error,robustness, compile time, time complexity...


\item \textbf{Generic}: General terms or pronouns that may refer to a entity but are not themselves informative, often used as connection words.

E.g model, approach, prior knowledge, them, it...

\end{itemize}



\subsection{Relation Category}
Relation link can not go beyond sentence boundary. We define 4 asymmetric relation types (\textit{Used-for}, \textit{Feature-of}, \textit{Hyponym-of}, \textit{Part-of}), together with 2 symmetric relation types (\textit{Compare}, \textit{Conjunction}).
\blue{B} always points to \red{A} for asymmetric relations

 \begin{itemize}
\item \textbf{Used-for}: \blue{B} is used for \red{A}, \blue{B} models \red{A}, \red{A} is trained on \blue{B}, \blue{B} exploits \red{A}, \red{A} is based on \blue{B}. E.g.
\begin{itemize}[label={}]
         \item The \blue{TISPER system} has been designed to enable many \red{text applications}.
         \item Our \blue{method} models \red{user proficiency}.
         \item Our \blue{algorithms} exploits \red{local soothness}.
\end{itemize}
\end{itemize}

\begin{itemize}
\item \textbf{Feature-of}: \blue{B} belongs to \red{A}, \blue{B} is a feature of \red{A}, \blue{B} is under \red{A} domain. E.g.
\begin{itemize}[label={}]
         \item \blue{prior knowledge} of the \red{model} 
         \item \blue{genre-specific regularities}  of  \red{discourse structure}
         \item \red{English text} in \blue{science domain}
\end{itemize}
\end{itemize}


\begin{itemize}
\item \textbf{Hyponym-of}: \blue{B} is a hyponym of \red{A}, \blue{B} is a type of \red{A}. E.g.
\begin{itemize}[label={}]
         \item \blue{TUIT} is a \red{software library}
         \item \red{NLP applications} such as \blue{machine translation} and \blue{language generation}
\end{itemize}
\end{itemize}


\begin{itemize}
\item \textbf{Part-of}: \blue{B} is a part of \red{A}... E.g.
\begin{itemize}[label={}]
         \item The \red{system} includes two models: \blue{speech recognition} and \blue{natural language understanding}
         \item We incorporate \blue{NLU module} to the \red{system}.
\end{itemize}
\end{itemize}

\begin{itemize}
\item \textbf{Compare}: Symmetric relation (use blue to denote entity). Opposite of conjunction, compare two models/methods, or listing two opposing entities. E.g.
\begin{itemize}[label={}]
         \item Unlike the \blue{quantitative prior}, the \blue{qualitative prior} is often ignored...
         \item We compare our \blue{system} with previous \blue{sequential tagging systems}...
\end{itemize}
\end{itemize}

\begin{itemize}
\item \textbf{Conjunction}: Symmetric relation (use blue to denote entity). Function as similar role or use/incorporate with. E.g.
\begin{itemize}[label={}]
         \item obtained from \blue{human expert} or \blue{knowledge base}
         \item NLP applications such as \blue{machine translation} and \blue{language generation}
\end{itemize}
\end{itemize}



\subsection{Coreference}
Two Entities that points to the same concept.
\begin{itemize}
\item \textbf{Anaphora and Cataphora}: 
\begin{itemize}[label={}]
         \item We introduce a \blue{machine reading system}... The \blue{system}...
         \item The \blue{prior knowledge} include...Such \blue{knowledge} can be applied to...
\end{itemize}
\item \textbf{Coreferring noun phrase}: 
\begin{itemize}[label={}]
         \item We develop a \blue{part-of-speech tagging system}...The \blue{POS tagger}...

\end{itemize}
\end{itemize}

\subsection{Notes}

\begin{enumerate}
\item Entity boundary annotation follows the ACL RD-TEC Annotation Guideline \cite{qasemizadeh2016acl}, with the extention that spans can be embedded in longer spans, only if the shorter span is involved in a relation.


\item Do not include determinators (such as ‘the’, ‘a’), or adjective pronouns (such as ‘this’,’its’, ‘these’, ‘such’) to the span. If generic phrases are not involved in a relation, do not tag them.


\item Do not tag relation if one entity is:
\begin{itemize}[]
\item Variable bound:

We introduce a neural based approach.. \textit{Its} benefit is...
\item The word \textit{which}:

We introduce a neural based approach, \textit{which} is a...
\end{itemize}
\item Do not tag coreference if the entity is

\begin{itemize}[]
\item Generically-used Other-ScientificTerm:

...advantage gained from \textit{local smoothness} which... We present algorithms exploiting \textit{local smoothness} in more aggressive ways...
\item Same scientific term but refer to different examples:

We use a \textit{data structure}, we also use another \textit{data structure}...
\end{itemize}
\item Do not label negative relations:

X is not used in Y or X is hard to be applied in Y

\end{enumerate}




==> S02-AnnotationExample.tex <==
\section{Annotation and Knowledge Graph Examples}
\label{sec:appendix}
Here we take a screen shot of the BRAT interface for an ACL paper in Figure~\ref{fig:ACL}.
% Following the annotation examples, 
We also attach the original figure of Figure 3 in Figure ~\ref{fig:SMT}. More examples can be found in the project website\footnote{\url{http://ssli.ee.washington.edu/tial/projects/sciIE/}}.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/NLP_example.pdf}
\vspace{-1em}
\caption{
Annotation example 1 from ACL 
}\label{fig:ACL}
\vspace{-1em}
\end{figure*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/CVPR_example.pdf}
% \vspace{-1em}
% \caption{
% Annotation example 2 from CVPR
% }\label{fig:CVPR}
% \vspace{-1em}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/ICASSP.pdf}
% \vspace{-1em}
% \caption{
% Annotation example 3 from ICASSP
% }\label{fig:ICASSP}
% \vspace{-1em}
% \end{figure*}

% \newpage
% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/ICML.pdf}
% \vspace{-1em}
% \caption{
% Annotation example 4 from ICML
% }\label{fig:ICML}
% \vspace{-1em}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/IJCAI.pdf}
% \vspace{-1em}
% \caption{
% Annotation example 4 from IJCAI
% }\label{fig:IJCAI}
% \vspace{-1em}
% \end{figure*}

\newpage

==> S03-KGexample.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth, keepaspectratio,clip]{sfigures/SMT.pdf}
\caption{
An example of our automatically generated knowledge graph centered on \textit{statistical machine translation}. This is the original figure of Figure \ref{fig:KG}.
}\label{fig:SMT}
\end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/CNN.pdf}
% \vspace{-1em}
% \caption{
% Automatically generated knowledge graph example centered on \textit{convolutional neural network} 
% }\label{fig:CNN}
% \vspace{-1em}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/CRF.pdf}
% \vspace{-1em}
% \caption{
% Automatically generated knowledge graph example centered on \textit{conditional random field} 
% }\label{fig:CRF}
% \vspace{-1em}
% \end{figure*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/NER.pdf}
% \vspace{-1em}
% \caption{
% Automatically generated knowledge graph example centered on \textit{named entity recognition} 
% }\label{fig:NER}
% \vspace{-1em}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth, keepaspectratio,clip]{sfigures/imagesegmentation.pdf}
% \vspace{-1em}
% \caption{
% Automatically generated knowledge graph example centered on \textit{image segmentation} 
% }\label{fig:IS}
% \vspace{-1em}
% \end{figure*}


==> tables/ablation_num_entities.tex <==
\begin{table}[h]
\footnotesize
\centering

\begin{tabular}{l r r r}
\toprule
Num. Entities & M=1 & M=2 & M=3 \\
\midrule
2 & 67.2 & 66.7 & 67.9 \\
3 & 61.8 & 59.1 & 62.6 \\
$[4, 6)$ & 53.4 & 58.3 & 56.7 \\
$[6, 12)$ & 60.3 & 61.0 & 62.2 \\
12+ & 50.0 & 49.1 & 56.3 \\
\bottomrule
\end{tabular}

\caption{TODO}
\label{tab:num_entities_ablation}
\end{table}



==> tables/confusion_matrix.tex <==
\begin{table}[h]

\begin{subtable}[t]{0.6\textwidth}
\begin{tabularx}{.4\textwidth}{c|c c c |}
 & PER & ORG & \multicolumn{1}{c}{GPE} \\
\hhline{----}
PER & 3167 \cellcolor[gray]{.8}& 91 & 34  \\
ORG & 98 & 744 \cellcolor[gray]{.8}& 27  \\
GPE & 80 & 41 & 1083 \cellcolor[gray]{.8} \\
\hhline{~---}
\end{tabularx}
\subcaption{Confusion matrix without coref.}
\label{tab:confusion_matrix:nocoref}

\end{subtable}
\begin{subtable}[t]{0.6\textwidth}
\begin{tabularx}{.4\textwidth}{c|c c c |}
 & PER & ORG & \multicolumn{1}{c}{GPE} \\
\hhline{----}
PER & 3185 \cellcolor[gray]{.8}& \textbf{65} & 31  \\
ORG & 90 & 750 \cellcolor[gray]{.8}& 27  \\
GPE & \textbf{54} & 34 & 1114 \cellcolor[gray]{.8} \\
\hhline{~---}
\end{tabularx}
\subcaption{Confusion matrix with coref.}
\label{tab:confusion_matrix:nocoref}
\end{subtable}

\caption{Confusion matrix for ACE entity extraction task for  \textit{PER}, \textit{ORG} and \textit{GPE}. \luanyi{added for camera ready}}
\label{tab:confusion_matrix}
\end{table}

==> tables/iteration.tex <==
\begin{table}[h]
\centering
{\footnotesize
\begin{tabular}{lll}
\toprule
\# of iterations & Coreference on NER & Relation on Relation \\
\midrule
$n=1$ & 85.9 & 57.6\\
$n=2$ & 86.4 & 59.2 \\
$n=3$ & \textbf{87.1} & \textbf{60.2} \\
$n=4$ & 86.7 & 58.8 \\
\bottomrule
\end{tabular}
}
\caption{F1 score of each layer on ACE development set for different number of iterations. $n=1$ indicates no propagation is made for the layer. \luanyi{coref on NER and relation on relation, confusing, not sure how to report}}

\label{tab:ablation:iteration}
\end{table}

==> tables/overlap_pr.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
%\setlength{\tabcolsep}{.25em}
\footnotesize
\centering

\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Non-overlapping} & \multicolumn{3}{c}{Overlapping} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& P & R & F1 & P & R & F1 \\
\midrule
\sys & 82.1 & 85.8 & \textbf{83.9} & 85.7 & 79.2 & \textbf{82.3} \\
\newcite{Wang2018NeuralSH} & 75.5 & 71.5 & 73.4 & 80.6 & 73.6 & 76.9 \\
\bottomrule

\end{tabularx}
\caption{NER results on sentences with and without an overlapping entity on ACE05-O.} 
\label{tab:overlap_pr}

\end{table}







% \begin{table}[h]

% \footnotesize
% \centering
% \begin{tabular}{lrr}

% \toprule
% & P & R & F1 \\
% \midrule
% Non-overlapping & 0.82 & 0.86 & 0.84 \\
% Overlapping & 0.86 & 0.79 & 0.82 \\
% \bottomrule

% \end{tabular}

% \caption{Results on sentences with and without an overlapping entity (ACE2005) \dwadden{TODO add comparison to SOTA.}}

% \label{tab:overlap_pr}


% \end{table}

==> tables/results_joint.tex <==
% Data sets on columns (flipped)

% Joint NER and REL

\begin{table}[h]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}

\begin{subtable}[t]{0.49\textwidth}
\footnotesize
\centering
\begin{tabular}{L{1.8cm}R{1.2cm}R{1.2cm}R{1.2cm}R{1.2cm}}
\toprule
\textbf{NER} & ACE04-J & ACE05-J & SciERC & WLPC \\
\midrule
Prev. SOTA & 81.8 & 83.6 & 64.2 & 78.0 \\
\sys & \textbf{87.4} & \textbf{88.4} & \textbf{65.4} & \textbf{79.7} \\
Abs. change & 5.6 & 4.8 & 1.2 & 1.7 \\
Pct. change & 6.8 & 5.7 & 1.9 & 2.2 \\
\bottomrule
\end{tabular}
\caption{Named entity extraction, test set F1.}
\label{tab:results_joint_ner}
\end{subtable}

\begin{subtable}[t]{0.49\textwidth}
\footnotesize
\centering
\begin{tabular}{L{1.8cm}R{1.2cm}R{1.2cm}R{1.2cm}R{1.2cm}}
\toprule
\textbf{REL} & ACE04-J & ACE05-J & SciERC & WLPC \\
\midrule
Prev. SOTA & 48.4 & 57.5 & 39.3 & *54.9 \\
\sys & \textbf{60.9} & \textbf{63.2} & \textbf{41.6} & \textbf{64.1} \\
Abs. change & 12.5 & 5.7 & 2.3 & *9.2 \\
Pct. change & 25.8 & 9.9 & 5.9 & *16.8 \\
\bottomrule
\end{tabular}
\caption{Relation extraction, test set F1.}
\label{tab:results_joint_rel}
\end{subtable}
\caption{Joint entity and relation extraction. \newline \emph{SOTA ACE2004-J}: \cite{miwa2016end}. \newline \emph{SOTA ACE2005-J}: \cite{zhang2017end}. \newline \emph{SOTA SciERC}: \cite{luan2018multi}. \newline \emph{SOTA WLPC}: \cite{Kulkarni2018AnAC} \newline * Compared to results of \cite{Kulkarni2018AnAC} with gold entity boudary given. \luheng{I'm wondering if it's possible to squeeze in the citations for each SoTA work in the Table ...}
}
\label{tab:results_joint}
\end{table}



% Data sets on rows

% \begin{table*}[t]
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \newcommand{\colindent}{\;}
% \setlength{\tabcolsep}{.25em}

% \footnotesize
% \centering

% \begin{tabularx}{\textwidth}{l c *{9}{Y}}
% \toprule
% & \multicolumn{3}{c}{Previous SOTA} & \multicolumn{2}{c}{\sys} & \multicolumn{2}{c}{Absolute change} & \multicolumn{2}{c}{Relative change} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
%  & & NER & REL & NER & REL & NER & REL & NER & REL \\    
% \midrule
% ACE2004-J & \cite{miwa2016end} & 81.8 & 48.4 & \textbf{87.4} & \textbf{60.9} & 5.6 & 12.5 & 6.8 & 25.8 \\
% ACE2005-J & \cite{zhang2017end} & 83.6 & 57.5 & \textbf{88.4} & \textbf{63.2} & 4.8 & 5.7 & 5.7 & 9.9 \\
% SciERC  & \cite{luan2018multi}  & 64.2 & 39.3 & \textbf{65.4} & \textbf{41.6} & 1.2 & 2.3 & 1.9 & 5.9 \\
% WLPC    & \cite{Kulkarni2018AnAC} & 78.0 & *54.9 / 79.0 & \textbf{79.7}  & *64.1 & 1.7 & *9.2 & 2.7 & *16.7 \\
% \bottomrule

% \end{tabularx}
% \caption{Joint entity and relation extraction. Test set F1. *\cite{Kulkarni2018AnAC} use gold entity candidates for all all relation models. We report results from their baseline model, and their best-performing model trained with additional features. We compare to their baseline model.}

% \label{tab:results_joint}


% \end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Old versions

% \begin{table*}[h]
% \centering
% {\footnotesize

% \begin{tabular}{llrrrr}
% \toprule
% Task & Previous SOTA paper & Previous SOTA & DynGraph & Absolute change & Relative change \\
% \midrule
% Ace 2004 non-overlapping NER & \cite{miwa2016end} & 81.8 & - & - & - \\
% Ace 2004 non-overlapping REL & \cite{miwa2016end} & 48.4 & - & - & - \\
% Ace 2004 overlapping NER & \cite{Wang2018NeuralSH} & 75.1 & - & - & - \\
% Ace 2005 non-overlapping NER & \cite{zhang2017end} & 83.6 & 88.4 & 4.8 & - \\
% Ace 2005 non-overlapping REL & \cite{zhang2017end} & 57.5 & 63.2 & 5.7 & - \\
% Ace 2005 overlapping NER & \cite{Wang2018NeuralSH} & 74.5 & 82.9 & 8.4 & - \\
% GENIA overlapping NER & \cite{Wang2018NeuralSH} & 75.1 & - & - & - \\
% Wet Lab NER & \cite{Kulkarni2018AnAC} & 78.03 & - & - & - \\
% Wet Lab REL & \cite{Kulkarni2018AnAC} & 54.85* & - & - & - \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results}
% \label{tab:summary}

% \end{table*}


% \begin{table*}[h]
% \begin{subtable}[t]{0.458\textwidth}
% % \centering
% {\footnotesize
% \begin{tabular}{llrrr}
% \toprule
% Task & Previous SOTA & & DynGraph & Absolute change \\
% \midrule
% ACE2004-J NER & \cite{miwa2016end} & 81.8 & - & - \\
% ACE2004-J REL & \cite{miwa2016end} & 48.4 & - & - \\
% ACE2005-J NER & \cite{zhang2017end} & 83.6 & 88.4 & 4.8 \\
% ACE2005-J REL & \cite{zhang2017end} & 57.5 & 63.2 & 5.7 \\
% SciERC NER & \cite{luan2018multi} & 64.2 & - & - \\
% SciERC REL & \cite{luan2018multi} & 39.3 & - & - \\
% WLPC NER & \cite{Kulkarni2018AnAC} & 78 & - & - \\
% WLPC REL & \cite{Kulkarni2018AnAC} & *54.9 & - & - \\
% \bottomrule
% \end{tabular}
% }

% \subcaption{Joint Named Entity and Relation Extraction}
% \label{tab:results_joint}

% \end{subtable}

% \begin{subtable}[t]{0.48\linewidth}
% % \centering
% {\footnotesize
% \begin{tabular}{llrrr}
% \toprule
% Task & Previous SOTA & & DynGraph & Absolute change \\
% \midrule
% ACE2004-O & \cite{Wang2018NeuralSH} & 75.1 & - & - \\
% ACE2005-O & \cite{Wang2018NeuralSH} & 74.5 & 82.9 & 8.4 \\
% GENIA & \cite{Wang2018NeuralSH} & 75.1 & - & - \\
% \bottomrule
% \end{tabular}
% }

% \subcaption{Overlapping Named Entity Extraction}
% \label{tab:results_nested}
% \end{subtable}

% \caption{Results \dwadden{TODO: align.}}
% \label{tab:results}
% \end{table*}



==> tables/results_overlapping.tex <==
% Overlapping REL
\begin{table}[h]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabular}{L{1.8cm}R{1.3cm}R{1.3cm}R{1.3cm}}
\toprule
\textbf{NER} & ACE04-O & ACE05-O & GENIA \\
\midrule
Prev. SOTA & 75.1 & 74.5 & 75.1 \\
\sys & \textbf{83.8} & \textbf{82.9} & \textbf{76.2} \\
Abs. change & 8.7 & 8.4 & 1.1 \\
Pct. change & 11.6 & 11.3 & 1.5 \\
\bottomrule
\end{tabular}
\caption{Overlapping entity extraction, test set F1. \newline \emph{SOTA all datasets}: \cite{Wang2018NeuralSH}.
}
\label{tab:results_overlap}
\end{table}


% \begin{table*}[t]
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \newcommand{\colindent}{\;}
% \setlength{\tabcolsep}{.25em}

% \footnotesize
% \centering

% \begin{tabularx}{\textwidth}{l c *{5}{Y}}
% \toprule
% & \multicolumn{2}{c}{Previous SOTA} & \sys & Absolute change & Relative change \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
%  & & NER & NER & NER & NER \\    
% \midrule
% ACE2004-O & \cite{Wang2018NeuralSH} & 75.1 & 83.8 & 8.7 & 11.6 \\
% ACE2005-O & \cite{Wang2018NeuralSH} & 74.5 & 82.9 & 8.4 & 11.3 \\
% GENIA  & \cite{Wang2018NeuralSH}  & 75.1 & 76.2 & 1.1 & 1.5 \\
% \bottomrule
% \end{tabularx}
% \caption{Overlapping entity extraction. Test set F1} \label{tab:results_overlap}

% \end{table*}


==> tables_old/data_coverage.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\linewidth}{l c *{3}{Y}}
    \toprule
     Statistics & \dataname & \semevalEnt & \semevalRel \\    
    \midrule
%    \#Docs   & 500 & 500 & 500\\
%   \#Entity types & 6 & 3 & -  \\
%   \#Relation types   & 7 & 2 & 6\\
   \#Entities  & 8089 & 9946 & 7483 \\
   \#Relations  & 4716 & 672 & 1595  \\
    \#Relations/Doc  & 9.4 & 1.3 & 3.2  \\
   \#Coref links& 2752 & - & -  \\
   \#Coref clusters& 1023 & - & -  \\
  \bottomrule
\end{tabularx}
\vspace{-1em}
\caption{Dataset statistics for our dataset \dataname\ and two previous datasets on scientific information extraction. All datasets annotate 500 documents.} %Comparison between other two information extraction tasks on scientific literature. Our dataset covers more tasks than previous ones. Our relation coverage is significantly higher than that of SemEval 2018.} 
  \label{tab:data}
  \vspace{-1em}
\end{table}

==> tables_old/exp_SemEval.tex <==
\begin{table*}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{.25em}
\footnotesize
\begin{tabularx}{\textwidth}{l c *{12}{Y}}
\toprule
    & \multicolumn{3}{c}{Span Indentification} & \multicolumn{3}{c}{Keyphrase Extraction} & \multicolumn{3}{c}{Relation Extraction} & \multicolumn{3}{c}{Overall}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule{11-13}
     Model & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1\\    
    \midrule
(Luan 2017)   & -   & -  & 56.9  & - & - & 45.3 & - &- &- & - &- &-\\
Best SemEval & 55   & 54   & 55  & 44 & 43 & 44 & 36 & 23 & \textbf{28} & 44 & 41 & 43\\
\sys\ & 62.2   & 55.4  & \textbf{58.6}  & 48.5   &  43.8  & \textbf{46.0} & 40.4 & 21.2 & 27.8 & 48.1 & 41.8 & \textbf{44.7} \\
\bottomrule
\end{tabularx}
% \vspace{-1em}
\caption{Results for scientific keyphrase extraction and extraction on SemEval 2017 Task 10, comparing with previous best systems.}
  \label{tab:semeval}
%   \vspace{-1em}
\end{table*}

==> tables_old/exp_ablations.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{.25em}
\footnotesize
\begin{tabularx}{\linewidth}{l c *{3}{Y}}
      \toprule
     %Task & \multicolumn{1}{c}{Single Task} & \multicolumn{1}{c}{w/ ner} & \multicolumn{1}{c}{w/ relation} & \multicolumn{1}{c}{w/ coref} & \multicolumn{1}{c}{w/o elmo}\\    
   Task &  Entity Rec. & Relation  & Coref.  \\
    %\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule{11-13} \cmidrule{14-16}
    %Metric & P & R & F1 & P & R & F1 &P & R & F1 &P & R & F1 & P & R & F1 \\  
    \midrule  
%Best Multitask   & 68.1 & 40.6 & 58.6 \\
%$-$\texttt{ELMo} & 65.2 & 34.5 & 52.6 \\
%\cmidrule(lr){1-4}
Multi Task (\sys) & 68.1 & 39.5 & 58.0 \\
    \midrule  
Single Task & 65.7 & 37.9 & 55.3 \\
$+$Entity Rec.      & -    & 38.9 & 57.1 \\
$+$Relation & 66.8 & -    & 57.6 \\
$+$Coreference    & 67.5 & 39.5 & -    \\
\bottomrule

\end{tabularx}
% \vspace{-1em}
\caption{Ablation study for multitask learning on \dataname\ development set. Each column shows results for the target task. %with ablations on different multitask setups.
}
  \label{tab:ablation}
%   \vspace{-1em}
\end{table}


% \begin{table*}[t]
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \setlength{\tabcolsep}{.25em}
% \footnotesize
% \begin{tabularx}{\textwidth}{l c *{15}{Y}}
%   %\begin{tabular}{l|lll|lll|lll|lll|lll}
%       \toprule
%      Task & \multicolumn{3}{c}{Single Task} & \multicolumn{3}{c}{w/ ner} & \multicolumn{3}{c}{w/ relation} & \multicolumn{3}{c}{w/ coref} & \multicolumn{3}{c}{w/o elmo}\\    
%     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule{11-13} \cmidrule{14-16}
%     Metric & P & R & F1 & P & R & F1 &P & R & F1 &P & R & F1 & P & R & F1 \\  
%     \midrule  
% ner & 66.1   & 65.2   & 65.7 & - & - & - & 67.8 & 65.8 & 66.8 & 69.2 & 65.8 & 67.5 & 66.3 & 64.1 & 65.2\\
% relation & 44.2 & 33.2 & 37.9 & 42.9 & 35.6 & 38.9 &- & - & -  & 45.5 & 36.6 & 40.6 & 39.7 & 30.5 & 34.5\\
% coref & 66.0 & 47.6 & 55.3 & 66.2 & 50.3 & 57.1 & 61.6 & 54.8 & 58.0 & - & - & - & 65.7 &43.8 &52.6\\
% \bottomrule
% \end{tabularx}
  
% \caption{Ablation study for multitask learning on the XXX development set. Each row shows results for the target task, with ablations on different multitask setups. We also show ablations by removing the ELMo embeddings.
% \luheng{say more, also change task names} \hanna{The table is hard to read and compare; I prefer to see the tasks in the top and the ablations as rows}}
%   \label{tab:ablation}
% \end{table*}


==> tables_old/exp_all_tasks.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering

\begin{subtable}{\linewidth}
\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
LSTM+CRF & 67.2   & 65.8   & 66.5  & 62.9   & 61.1   & 62.0   \\
LSTM+CRF+ELMo & 68.1   & 66.3   & 67.2  & 63.8   & 63.2   & 63.5   \\
\mb({\pipeline}) & 66.7   & 65.9   & 66.3  & 60.8   & 61.2   & 61.0   \\
\mb     & 64.3   & 68.6   & 66.4  & 60.6   & 61.9   & 61.2   \\
\mb+\elmo & 67.5   & 66.3   & 66.9  & 63.5   & 63.9   & 63.7  \\
%\cmidrule(lr){1-7}
\sys\ & 70.0   & 66.3  & \textbf{68.1}  & 67.2   &  61.5  & \textbf{64.2}  \\
\bottomrule
\end{tabularx}
\caption{Entity recognition.}\label{tab:ner}
\end{subtable}

\begin{subtable}{\linewidth}
\begin{tabularx}{\columnwidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
\mb({\pipeline})  & 34.2   & 33.7   & 33.9  & 37.8   & 34.2   & 35.9  \\

\mb   & 37.3   & 33.5   & 35.3  & 37.1   & 32.2   & 34.1  \\
\mb+\elmo & 38.5   & 36.4   & 37.4  & 38.4   & 34.9   & 36.6  \\
%\cmidrule(lr)
\sys\ & 45.4   & 34.9  & \textbf{39.5}  & 47.6   &  33.5  & \textbf{39.3}  \\
\bottomrule
 \end{tabularx}
 \caption{Relation extraction.}\label{tab:relation}
 \end{subtable}
 
 \begin{subtable}{\linewidth}
 \begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     Model & P & R & F1 & P & R & F1 \\    
    \midrule
{\coref}     & 59.4   & 52.0   & 55.4  & 60.9   & 37.3   & 46.2    \\
\sys & 61.5   & 54.8   & \textbf{58.0}  & 52.0 & 44.9 & \textbf{48.2} \\
\bottomrule
\end{tabularx}
\caption{Coreference resolution. 
}\label{tab:coref}
\end{subtable}
% \vspace{-1em}
\caption{
Comparison with previous systems on the development and test set for our three tasks.
For coreference resolution, we report the average P/R/F1 of MUC, $\text{B}^3$, and $\text{CEAF}_{\phi_4}$ scores. %\newcite{Pradhan2012CoNLL2012ST}.
}
\label{tab:alltasks}
% \vspace{-1em}
\end{table}

==> tables_old/exp_coreference.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     Model & P & R & F1 & P & R & F1 \\    
    \midrule
E2E Coref      & 59.4   & 52.0   & 55.4  & 60.9   & 37.3   & 46.2    \\
\sys\ & 61.5   & 54.8   & \textbf{58.0}  & 52.0 & 44.9 & \textbf{48.2} \\
\bottomrule
\end{tabularx}
\caption{Results for coreference resolution. We report average F1 \luheng{cite} for simplicity.}\label{tab:coref}
\end{table}


==> tables_old/exp_keyphrase_extraction.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
M\&B \texttt{pipeline}  & 66.7   & 65.9   & 66.3  & 60.8   & 61.2   & 61.0   \\
M\&B \texttt{joint}     & 64.3   & 68.6   & 66.4  & 60.6   & 61.9   & 61.2   \\
M\&B+\texttt{ELMo} & 67.5   & 66.3   & 66.9  & 63.5   & 63.9   & 63.7  \\
%\cmidrule(lr){1-7}
\sys\ & 70.0   & 66.3  & \textbf{68.1}  & 64.4   &  64.7  & \textbf{64.5}  \\
\bottomrule
\end{tabularx}
\caption{Results for scientific keyphrase extraction in terms of labeled precision, recall and F1 on the development and test set. }\label{tab:ner}
\end{table}

==> tables_old/exp_relation_extraction.tex <==
\begin{table}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\columnwidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
M\&B \texttt{pipeline}  & 34.2   & 33.7   & 33.9  & 37.8   & 34.2   & 35.9  \\

M\&B \texttt{joint}    & 37.3   & 33.5   & 35.3  & 37.1   & 32.2   & 34.1  \\
M\&B+\texttt{ELMo} & 38.5   & 36.4   & 37.4  & 38.4   & 34.9   & 36.6  \\
%\cmidrule(lr)
\sys\ & 45.5   & 36.6  & \textbf{40.6}  & 47.9   &  33.8  & \textbf{39.6}  \\
\bottomrule
 \end{tabularx}
\caption{Results for scientific relation extraction in terms of labeled P/R/F1 on development and test set.}\label{tab:relation}
\end{table}

